$2 * n$ is better than $n^2$: Decomposing Event Coreference Resolution into Two Tractable Problems

Event Coreference Resolution (ECR) is the task of linking mentions of the same event either within or across documents. Most mention pairs are not coreferent, yet many that are coreferent can be identified through simple techniques such as lemma matching of the event triggers or the sentences in which they appear. Existing methods for training coreference systems sample from a largely skewed distribution, making it difficult for the algorithm to learn coreference beyond surface matching. Additionally, these methods are intractable because of the quadratic operations needed. To address these challenges, we break the problem of ECR into two parts: a) a heuristic to efficiently filter out a large number of non-coreferent pairs, and b) a training approach on a balanced set of coreferent and non-coreferent mention pairs. By following this approach, we show that we get comparable results to the state of the art on two popular ECR datasets while significantly reducing compute requirements. We also analyze the mention pairs that are "hard" to accurately classify as coreferent or non-coreferent. Code at https://github.com/ahmeshaf/lemma_ce_coref

==> reviews.tex <==
ACL 2023 Reviews for Submission #2383
============================================================================ 

Title: Two times n is better than n-squared: Decomposing Event Coreference Resolution into Two Tractable Problems
Authors: Shafiuddin Rehan Ahmed, Abhijnan Nath, James H. Martin and Nikhil Krishnaswamy
============================================================================
                            META-REVIEW
============================================================================ 

Comments: The paper proposes a technical contribution, i.e., decomposing event coreference resolution into two steps: rule-based pruning step and training on the output of the first step. This essentially reduces computing time by a lot (as not all potential examples have to be considered). Rev1 and rev3 are very positive, but rev2 points out some methodological problems that I find the authors don't address in the best way. Namely the system inconsistency between training and inference time, and wether using all the positive examples would have led to SOTA results. Their response focus on the factual info that rev2 got wrong.

============================================================================
                            REVIEWER #1
============================================================================

What is this paper about and what contributions does it make?
---------------------------------------------------------------------------
In this paper the authors contribute to event coreference resolution research by proposing a lemma-based heuristic for filtering out true negative mentions as a preprocessing step. This step is targeted at reducing the number of mention pairs that need to be considered for mention clustering, and thereby also substantially reduces computational cost. Mentions are then fed into a transformer-based cross-encoding system for prediction.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
One substantial benefit is I found this paper to be exceptionally clear for the most part. The problem is presented very cleanly, and the steps taken as well are thoroughly explained in a very logical way. 

The method is simple and does not achieve SOTA performance on the task, but nevertheless introduces a strong baseline and jumping-off point for future work.

The qualitative error analysis carried out is extensive, detailed, and useful.

Overall and simply put, the paper is solid and makes a reasonable incremental contribution to the literature in this area.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
The core concept in this paper, namely pruning the possible space of coreferent mentions before performing an embedding-based pairwise classification, is fundamentally already presented in Held et al. 2021. 

As a result, I would have loved to see error analysis not just on its own, but in relation to Held et al. 2021. Are there instances or categories of your system gets right that they get wrong?
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
Question A: I'm somewhat confused by section 7.2 and feel that it is essential to clarify this piece in the final version of the paper. In what way do Held et al. 2021 use an oracle coreference scorer after their pruning step? Essentially the issue here, is perhaps the authors need to better contextualize their results so readers can understand how we should interpret the performance of this method in relation to existing ones. The non-oracle versions of LH are all straightforwardly worse than Held et al. 2021. Is there some important way I'm missing that we should see LH_oracle as directly comparable to Held?
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                               Soundness: 4
                 Excitement (Long paper): 4
                     Reviewer Confidence: 4
     Recommendation for Best Paper Award: No
                         Reproducibility: 5
                        Ethical Concerns: No


============================================================================
                            REVIEWER #2
============================================================================

What is this paper about and what contributions does it make?
---------------------------------------------------------------------------
This paper presents a new hybrid approach for event coreference
resolution (ECR), using heuristic rules (based on string and synonym
matching) to prune down the number of non-coreference pairs to
consider during training. This makes the overall approach more
tractable, and the learning phase possibly easier as the distribution
of positive and negative mention pairs is less unbalanced. The neural
model is a transformer-based mention pair cross-encoder, similar to
those used in previous work but "symmetrized" and trained directly on
the outputs of the rule-based component. Experiments are carried on
two dataset, namely: ECB+, which is the main benchmark for this task,
and the newer and more specific Gun Violence Corpus (GVC). Results are
competitive with the SOTA (in this case, Held et al. 2021), though
only when using oracle rules, and time complexity is linear in the
number of mentions.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
- Motivations are very clear, as ECR remains a very challenging task
  even for recent neural-based models, and most models are not
  tractable.

- The proposed approach is very simple and leads to tractable models

- The paper is well written and easy to follow
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
- The paper claims that the time complexity of the approach is 2*N
  (with N, the number of mentions), but this is never completely shown
  either theoretically or empirically.

- There are a number of weaknesses in the approach:

  -- there seems to be an important discrepancy between how the model
    is trained and the way it is used at inference time. Put it
    simply, the cross encoder is trained to mitigate some of the
    errors of the heuristic rules, but at inference time only the
    pairs considered coreferential by the rules are passed on to the
    encoder (excluding many possible false negative). 

  -- As far as I understand, not all all positive pairs from the
    training data are using between training (but only those), which
    seems like a waste.

  -- the use of a symmetric cross-encoder is not very well motivated,
    neither from a linguistic point of view (as some cases, likely to
    be missed by the heuristics, are instances of anaphora, hence by
    definition asymmetrical), nor from an empirical perspective (as
    there is no empirical comparison with a non-symmetric encoder).

  -- the overall design of the system is motivated by error analysis of
    the heuristic rules made on the training, dev, but also the test
    data (!)
  

- Overall, the experimental part of the paper is not entirely
  compelling.

  -- The reported results for the proposed approach are substantially
    below the SOTA, unless oracle rules are used.

  -- The approach should probably be compared to standard sub-sampling
    techniques.
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                               Soundness: 2
                 Excitement (Long paper): 2
                     Reviewer Confidence: 3
     Recommendation for Best Paper Award: No
                         Reproducibility: 4
                        Ethical Concerns: No


============================================================================
                            REVIEWER #3
============================================================================

What is this paper about and what contributions does it make?
---------------------------------------------------------------------------
This paper proposes an efficient method for event coreference resolution which reduces complexity by breaking down the task in two phases, the first of which deploys a quasi-easy-first heuristic strategy based on a careful analysis of the easy vs difficult cases, followed by a more traditional classifier. The system achieves a substantial reduction in computation, with about 4 percentage points loss in performance in the ECB dataset, but much more substantial in the GVC dataset.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
1. This is a very well written paper discussing an extremely well engineered system

2. The chosen approach is based on an extensive analysis of the task, a rarity these days.

3. The empirical methodology is of a high quality
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
1. The main problem I have is that although the method is very clever, the model in the end doesn't really push forward the state of the art in event coreference resolution - it tells us how to trade accuracy for speed

2. but the loss of accuracy seems too high to me, particularly in GVC
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
I don't really have any questions, the paper is pretty clear

Question A:

Question B:

Question C:
---------------------------------------------------------------------------


Missing References
---------------------------------------------------------------------------
One serious omission: the `easy first' approach to coreference was actually invented by Breck Baldwin in his CogNIAC system 
https://aclanthology.org/W97-1306/
---------------------------------------------------------------------------


Typos, Grammar, Style, and Presentation Improvements
---------------------------------------------------------------------------
No problem
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                               Soundness: 4
                 Excitement (Long paper): 3
                     Reviewer Confidence: 3
     Recommendation for Best Paper Award: No
                         Reproducibility: 4
                        Ethical Concerns: No


